ChatGPT: A Meta-Analysis after 2.5 Months

ChatGPT, a chatbot developed by OpenAI, has gained widespread popularity and media attention since its release in November 2022. However, little hard evidence is available regarding its perception in various sources. In this paper, we analyze over 300,000 tweets and more than 150 scientific papers to investigate how ChatGPT is perceived and discussed. Our findings show that ChatGPT is generally viewed as of high quality, with positive sentiment and emotions of joy dominating in social media. Its perception has slightly decreased since its debut, however, with joy decreasing and (negative) surprise on the rise, and it is perceived more negatively in languages other than English. In recent scientific papers, ChatGPT is characterized as a great opportunity across various fields including the medical domain, but also as a threat concerning ethics and receives mixed assessments for education. Our comprehensive meta-analysis of ChatGPT's current perception after 2.5 months since its release can contribute to shaping the public debate and informing its future development. We make our data available.

==> sections/background.tex <==
\section{Background}
We take inspiration from three recent supervised (reference-free; \type{3})
metrics: \xmoverscore~\citep{Zhao2020OnTL},
\distilscore~\citep{Reimers2020MakingMS}, and
\sentsim~\citep{Song2021SentSimCS}. Below, we review key aspects of them, and
show where supervision plays a role.

\subsection{\xmoverscore}\label{sec:xmover}
Central to \xmoverscore{} is the use of Word Mover's Distance (WMD) as a
similarity  between two sentences~\citep{Zhao2020OnTL}. WMD and further
enhancements are discussed below.

\paragraph{WMD}\label{par:wmd}
WMD is a distance function that compares sentences at the token
level~\citep{Kusner2015FromWE}, by leveraging word embeddings which in
\xmoverscore{}'s case come from \mbert~\citep{devlin2018bert}. From a source
sentence $x$ and an MT hypothesis $y$, WMD constructs a  \emph{distance matrix}
$\mathbf{C}\in\mathbb{R}^{|x|,|y|}$, where $\mathbf{C}_{ij}$ is the distance
between two word embeddings, $\mathbf{C}_{ij}=\|\embed(x_i) - \embed(y_j)\|$;
$x_i,y_j$ index respective words in $x$, $y$. WMD uses this distance matrix to
compute the similarity of the two sentences. This  can be defined as the linear
programming problem
\begin{equation}\begin{split}
  \wmd(x,y)&= \min_\mathbf{F}
    \sum_{i=1}^{|x|}\sum_{j=1}^{|y|}\mathbf{F}_{ij}\mathbf{C}_{ij},
\end{split}\end{equation}
where $\mathbf{F}\in\mathbb{R}^{|x|,|y|}$ is an \emph{alignment matrix} with
$\mathbf{F}_{ij}$ denoting how much of word $x_i$ travels to word $y_j$.
Additional constraints prevent it from becoming a zero matrix.

\paragraph{Vector space remapping}
\citet{Zhao2020OnTL}, akin to similar earlier and subsequent work
\citep{Cao2020Multilingual,schuster-etal-2019-cross}, argue that the
monolingual subspaces of \mbert{} are not well aligned. As a remedy, they
investigate linear projection methods which post-hoc improve cross-lingual
alignments. We refer to this approach as vector space \emph{remapping}.
\xmoverscore{} explores two different remapping approaches, CLP and UMD\@. They
both leverage parallel data on sentence-level from which they extract
word-level alignments using \fastalign{}, which are then used for remapping. We
give more details in the Appendix~\ref{sec:remapping}.

\paragraph{Language Model}
\xmoverscore{} linearly combines WMD with the perplexity of a \gpt{} language
model~\citep{Radford2019LanguageMA}. Allegedly this penalizes ungrammatical
translations. This updates \xmoverscore{}s scoring function to
\begin{equation}\label{eq:lm-combine}
  \begin{split}
    \m(x,y) ={}& \wxling\wmd(x,y)+ \wlm\lm(y).
  \end{split}
\end{equation}
Here, $\wxling$, $\wlm$ are weights for the cross-lingual WMD and LM components
of \xmoverscore{}.

\subsection{\distilscore{}}\label{sec:distill}
\citet{Reimers2020MakingMS} show that the cosine between multilingual sentence
embeddings captures semantic similarity and can be used to assess cross-lingual
semantic textual similarity. Their approach to inducing embedding models is
based on multilingual knowledge distillation. We refer to this metric as
\distilscore. Their approach requires supervision at multiple levels. First,
parallel sentences are needed to induce multilingual models, and second, NLI
and STS corpora are required to induce teacher embeddings in the source
language.

\subsection{\sentsim{}}\label{sec:sentsim}
A key difference between \xmoverscore{} and \distilscore{} is that one approach
is based on word- and the other on sentence embeddings.
\citet{Song2021SentSimCS} and \citet{kaster-etal-2021-global} show that
combining approaches based on word-level and sentence-level representations can
substantially improve metrics. The metric of \citet{Song2021SentSimCS}, which
is called \sentsim, combines supervised \distilscore{} with one of two word
embedding-based metrics. The first one is quite similar to \xmoverscore{}, as
it is also based on WMD\@. The other one is a multilingual variant of
\bertscore{}~\citep{Zhang2020BERTScoreET}.


==> sections/limitations.tex <==
\section{Limitations}\label{sec:limitations}
Limitations of our metrics include (1) \emph{algorithmic inefficiency}, (2)
\emph{resource inefficiency}, (3) the brittleness of unsupervised MT systems in
certain situations, and (4) issues of adversarial robustness.

(1) Some of the components of \metric[wrd] (mainly the MT system) have high
computational costs. For example, \xmoverscore{} and \sentsim[BERTScore] take
less than 30 seconds to score 1000 hypotheses on an Nvidia V100 GPU\@.
\metric[wrd], on the other hand, takes over 2.5 minutes. This algorithmic
inefficiency trades off with our sample efficiency, by which we did not use any
supervision signals. In future work, we aim to experiment with efficient MT
architectures  to reduce computational costs
\citep{kamal-eddine-etal-2022-frugalscore,Grunwald2022CanWD}.

(2) Similarly to \xmoverscore{}, \monotransquest{} or \sentsim[], our metrics
use high-quality encoders such as \mbert{}, which are not only memory and
inference inefficient but also leverage large monolingual resources. Future
work should thus not only investigate using smaller \mbert{} models but also
models that leverage smaller amounts of monolingual resources.
\citet{wang-etal-2020-extending}, for example, propose a competitive LSTM-based
approach that completely forgoes monolingual resources and instead uses small
parallel corpora (i.e., a few hundred parallel sentences as a weak supervision
signal). Similarly, we give a recipe for improving \mbert{} for unseen
languages using limited amounts of parallel data in
Appendix~\ref{sec:finetune}.

(3)  Using unsupervised MT approaches, as we do via pseudo references, may be
less effective for truly low-resource languages
\citep{marchisio-etal-2020-unsupervised}. However, this remains a very active
research field with a constant influx of more powerful solutions
\citep{ranathunga2021neural,sun2021unsupervised}.

(4) As indicated in Sections~\ref{sec:preliminary}~and~\ref{sec:analysis}, our
mined pseudo-parallel data tends to contain factual inconsistencies such as
``Uruguay was seventh'' vs.\ (a translation of) ``Russia was second''. As a
consequence, our induced metrics may be less robust than existing metrics
\citep{Chen2022MENLIRE,rony-etal-2022-rome}. An approach to address this
inconsistency would be to retain only high probability aligned words in
parallel sentences (recall that we infer word-level parallel data from
sentence-level parallel data).


==> sections/methods.tex <==
\section{Methods}
In this section, we introduce our fully unsupervised metric \metric{}.
\metric{} builds upon the existing metrics \xmoverscore, \distilscore, and
\sentsim{}, but eliminates all supervision signals and instead leverages the
dualities shown in Figure~\ref{fig:self}. In particular, we mine
pseudo-parallel data from unsupervised metrics, which we use (iteratively) to
(a) rectify deficient vector spaces (for \xmoverscore) and to (b) train
unsupervised MT systems which can generate pseudo-references (as
pseudo-references are in the same language as the hypothesis, this eliminates
problems of cross-lingual deficiency). Furthermore, we use pseudo-parallel data
to (c) induce an unsupervised sentence embedding model analogous to
\distilscore, which we can then (d) integrate with the unsupervised word based
model analogous to \sentsim{}. We now give details.

\subsection{\metric[wrd]}\label{sec:wmd}
\xmoverscore{} uses sentence-parallel data to extract word pairs for vector
space remapping. (i) We replace this parallel data with pseudo-parallel
data.\footnote{To extract the word pairs from the sentence-parallel data,
\xmoverscore{} uses \fastalign~\citep{Dyer2013ASF}, but since this depends
directly on how well sentences are aligned, we first replace it with
unsupervised \awesomealign~\citep{Dou2021WordAB} which only relies on
pre-trained language models.} (ii) In addition, we use pseudo-references to
address the issue of deficient vector spaces. We now give details on (i) and
(ii) below.

\begin{figure}[tb]
  \centering
  \scriptsize
  \input{xmover-components.pdf_tex}
  \caption{\metric[wrd] with pseudo
  references (left), unsupervised remapping (middle) and a LM
  (right).}%
  \label{fig:xmover-components}
\end{figure}

\paragraph{Efficient WMD Pseudo-Parallel Data  Mining}
Metrics such as \xmoverscore{} could in principle be used for pseudo-parallel
corpus mining since they can compare arbitrary sentences. However, when
WMD-based metrics are scaled to corpus mining, algorithmic efficiency problems
arise: (a) the computational complexity of WMD scales cubically with sentence
length~\citep{Kusner2015FromWE}; (b) to compare $m$ source to $m$ target
sentences, $m^2$ WMD invocations are necessary, which quickly becomes
intractable. Thus, we explore ways to improve the performance of WMD to mine
efficiently. In particular, \citet{Kusner2015FromWE} define a linear
approximation of WMD called \emph{word centroid distance}  (WCD) and a mining
algorithm that first sorts all target samples according to their WCD\@ to a
given query and computes exact WMD for the $k$ nearest neighbors. We use this
algorithm for efficient WMD-based pseudo-parallel data mining.

In our work, we apply this approach \emph{iteratively} (cf.\
Figure~\ref{fig:self}): we start out with an initial WMD metric (based on
\mbert{}), obtain \emph{sentence-level} pseudo-parallel data with it via the
efficient approximation algorithm described, and obtain a dictionary of word
pairs from unsupervised \awesomealign{} from the sentence pseudo-parallel data.
We use the pseudo-parallel word pairs with UMD and CLP to remap \mbert{}. From
this, we obtain a better WMD metric; then we iterate.


\paragraph{Pseudo References}
Apart from remapping, pseudo-parallel data could be used to overcome problems
of deficient vector spaces in other ways. Specifically, we want to mine enough
pseudo-parallel data to train an unsupervised MT system to translate source
sentences into the target language to create \emph{pseudo
references}~\citep{albrecht-hwa-2007-regression,gao-etal-2020-supert,Fomicheva2020MultiHypothesisMT}.
This would allow for a comparison with the hypothesis in the target language,
similar to reference-based metrics, circumventing alignment problems in
multilingual embeddings. This approach updates \metric[wrd] to
\begin{equation}
  \begin{split}\label{eq:wmd-combine}
    \m(x,y,y') ={}& \wxling\wmd^{(n)}(x,y) + \wlm\lm(y) \\ &+ \wpseudo\wmd(y,y'),\\
  \end{split}
\end{equation}
where $n$ denotes the iterations of remapping, and $\wpseudo$ is a new weight
to control the influence of the pseudo reference $y'$. All components of
\metric[wrd] are illustrated in Figure~\ref{fig:xmover-components}.



\subsection{\metric[snt]}\label{sec:cos}
Besides a word-based metric, we use pseudo-parallel data to induce an
unsupervised \emph{sentence level} metric, $\metric[snt]=\cos(x,y)$, based on
the cosine similarity between sentence embeddings. One could, similarly to
\distilscore{}, perform knowledge distillation but since our initial
experiments showed that this doesn't work well with pseudo-parallel data, we
chose another approach.

\paragraph{Contrastive Learning}
We explore contrastive learning for unsupervised \emph{multilingual} sentence
embedding induction, which has recently been successfully used to train
unsupervised \emph{monolingual} sentence embeddings~\citep{gao2021simcse}. In
our context, the basic idea  is to pull semantically close sentences together
and to push distant sentences apart in the embedding space. Let $x_i$ and $y_i$
be the embeddings of two sentences that are semantically related and $N$ an
arbitrary batch size. The training objective for this pair can be formulated as
\begin{equation}
  L_i=-\log\frac{\exp{(\frac{\cos(x_i, y_i)}{\tau}})}
    {\sum^N_{j=1,j\neq i}\exp({\frac{\cos(x_i, y_j)}{\tau}})},
\end{equation}
where $\tau$ is a temperature hyperparameter that can be used to either amplify
or dampen the assessed distances. For each sentence $x_i$, all remaining
sentences $y_{j\neq i}$ in the current batch  should be pushed apart in the
embedding space. For positive sentences that should be pulled together, we
again use pseudo-parallel sentence pairs. Since noisy data is beneficial for
contrastive learning~\citep{gao2021simcse}, we expect this paradigm to work
well with pseudo-parallel data. We use pooled \xlmr{} embeddings as sentence
representations, and, as with unsupervised remapping, we experiment with
multiple iterations of successive mining and sentence embedding induction
operations.

\paragraph{Ratio Margin Pseudo-Parallel Data  Mining}
As \metric[snt] is based on sentence embeddings, we cannot use the WMD-based
mining algorithm to obtain pseudo-parallel sentences since it requires access
to word-level representations. An alternative would be to just use cosine
similarity for mining, but that approach is susceptible to noise in the
data~\citep{Artetxe2019MarginbasedPC}. Instead, we follow
\citet{Artetxe2019MarginbasedPC} and use a ratio margin function defined as
\begin{equation}
  \margin(x, y)=\frac{%
    \cos(x,y)
  }{%
    \sum\limits_{z\in N_x}\frac{\cos(x,z)}{2k} +
    \sum\limits_{z\in N_y}\frac{\cos(y,z)}{2k}
  },
\end{equation}
where $N_x$ and $N_y$ are the $k$ nearest neighbors of sentence embeddings $x$
and $y$ in the respective language. Informally, this ratio margin function
divides the cosine similarities of the nearest neighbor by the average
similarities of the neighborhood.

\subsection{\metric[wrd\,$\oplus$\,snt]}\label{sec:ensembles}
Inspired by \sentsim{}, which combines word and sentence embeddings, we
similarly ensemble \metric[wrd] and \metric[snt]. We refer to this final metric
as \metric{} $\:\:=$ \metric[wrd\,$\oplus$\,snt] with two new weights $\wwmd$
and $\wcos=1-\wwmd$:
\begin{equation}
  \begin{split}
    \metric(x,y) ={}& \wwmd\operatorname{\metric[wrd]}(x,y)\\
    &+ \wcos\operatorname{\metric[snt]}(x,y).
  \end{split}
\end{equation}


==> sections/unused.tex <==
\section{Vector Space Remapping}\label{sec:remapping}
\citet{Zhao2020OnTL} explore two different remapping approaches for
\xmoverscore, which are defined as follows:
\begin{description}
  \item[Procrustes alignment] \citet{Mikolov2013ExploitingSA} propose to
    compute a linear transformation matrix $\mathbf{W}$ which can be used to
    map a vector $x$ of a source word into the target language subspace by
    computing $\mathbf{W}x$. The transformation can be computed by solving the
    problem \begin{equation} \min_\mathbf{W}||\mathbf{WX} - \mathbf{Y}||_2.
    \end{equation} Here $\mathbf{X}, \mathbf{Y}$ are matrices with embeddings
    of source and target words, respectively, where the tuples $(x_i,y_i)\in
    \mathbf{X}\times \mathbf{Y}$ come from parallel word pairs. \xmoverscore{}
    constrains $\mathbf{W}$ to be an orthogonal matrix such that
    $\mathbf{W}^{\intercal}\mathbf{W}=\mathbf{I}$, since this can lead to
    further improvements~\citep{Xing2015NormalizedWE}. \citet{Zhao2020OnTL}
    call this remapping Linear Cross-Lingual Projection remapping (CLP).

  \item[De-biasing] The second remapping method of \xmoverscore{} is
    rooted in the removal of biases from word embeddings.
    \citet{Dev2019AttenuatingBI} explore a bias attenuation technique called
    Universal Language Mismatch-Direction (UMD). It involves a bias vector
    $v_B$, which is supposed to capture the bias direction. For each word
    embedding $e$, an updated word embedding $e'$ is computing by subtracting
    their projections onto $v_B$, as in \begin{equation} e' = e - (e\cdot
    v_B)v_B, \end{equation} where $\cdot$ is the dot product. To obtain the
    bias vector $v_B$, \citet{Dev2019AttenuatingBI} use a set $\mathcal{E}$ of
    word pairs that should be de-biased (e.,g.\ \emph{man} and \emph{woman}).
    The subtractions of the embeddings of the words in each pair are then
    stacked to form a matrix $\mathbf{Q}$, and the bias vector $v_B$ is its
    top-left singular vector. \citet{Zhao2020OnTL} use the same approach for
    \xmoverscore{}, but $\mathcal{E}$ instead consists of parallel word pairs.
\end{description}

\citet{Zhao2020OnTL} show that these remapping methods lead to substantial
improvements of their \xmoverscore{} metric (on average, up to 10 points in
correlation). The required parallel word pairs were extracted from sentences of
the EuroParl corpus~\citep{Koehn2005EuroparlAP} using the
\fastalign{}~\citep{Dyer2013ASF} word alignment tool. The best results were
obtained when remapping on 2k parallel sentences.


\section{Filtering}\label{sec:filtering}
Since large corpora tend to include low-quality data points, we follow
\citet{Artetxe2019MarginbasedPC} and \citet{Keung2021UnsupervisedBM} and apply
three simple filtering techniques. We first remove all sentences from each
monolingual corpus for which the \fasttext{} language identification
tool~\citep{joulin2016bag} predicts a different language. We then filter all
sentences which are shorter than 3 tokens or longer than 30 tokens. As the last
step, we discard sentence pairs sharing substantial lexical overlap, which
prevents degenerate alignments of, e.g., proper names. We remove all sentence
pairs for which the Levenshtein distance detects an overlap of over 50\%.

\section{Fine-Tuning on Parallel Data}\label{sec:finetune} 
\begin{figure}[tb]
  \centering
    \input{finetune.pgf}
    {\footnotesize
      \begin{tabular}{llllll}
        \toprule
            & ---   & 10k   & 20k   & 30k   & 200k\\
        \midrule
        Avg & 40.60 & 42.95 & 44.42 & 45.17 & \textbf{46.57}\\
        \bottomrule
      \end{tabular}
    }
    \caption{\pearson{} correlations on MLQE-PE for \metric[wrd\,$\oplus$\,snt]
    when fine-tuning on limited amounts of parallel data. We explore sample
    sizes of 10k, 20k, 30k, and 200k.}%
    \label{fig:finetune}
\end{figure}
To examine whether and by how much we can further improve our metrics using
forms of supervision, we experiment with a fine-tuning step on \emph{parallel
sentences} and treat self-learning on pseudo-parallel data as
pre-training~\citep{He2020RevisitingSF}. We use the parallel data to fine-tune
the contrastive sentence embeddings of \metric[snt] and the MT system of
\metric[wrd], which is responsible for generating pseudo references. Further,
we also compute new remapping matrices for \metric[wrd]. Since CLP is superior
to UMD when parallel data is used (see Section~\ref{par:remapping}), we compute
these remapping matrices using CLP instead of UMD\@. To assess how different
amounts of parallel sentences affect performance, we fine-tune our metrics on
10k, 20k, 30k, and 200k parallel sentences. We use
WikiMatrix~\citep{Schwenk2021WikiMatrixM1} and the Nepali Translation Parallel
Corpus~\citep{Duwal2019EffortsIT} to obtain parallel sentences.

\pearson{} correlations with human judgments for individual and averaged
language pairs are shown in Figure~\ref{fig:finetune}; we focus on MLPQE-PE,
where our metrics performed worst. Overall, introducing parallel data into the
training process consistently improves performance for the majority of language
directions; more parallel data leads to better results. The relatively biggest
improvements are achieved for the si-en language direction, which is in
accordance with our discussion above. When fine-tuning with 30k parallel
sentences, the performance of our metrics is roughly on par with the \sentsim{}
variants (see Table~\ref{tab:correlations}). With 200k parallel sentences, our
metrics clearly outperform \sentsim{}, which uses millions of parallel
sentences and NLI data as supervision signals.

\section{Hyperparameters}\label{sec:hyperparameters}
For efficient WMD pseudo-parallel mining, we set $k=20$ for remapping, and
$k=1$ for training \mbart. For ratio-margin-based pseudo-parallel mining, we
use $k=5$.
%
With regard to training \metric[snt], we follow \citet{gao2021simcse}, and
iteratively train \xlmr{} for one training epoch with a learning rate of 5e-5,
a batch size of 256, and a temperature coefficient of $\tau=0.05$ utilizing the
AdamW optimizer~\citep{Loshchilov2019adamw}.
%
Fine-tuning of \mbart{} was performed for three epochs with a batch size of
four and using the same learning rate of 5e-5 as well as AdamW optimizer.

We decided to continue using \mbert{} in \metric[wrd] for two reasons. Firstly,
we want \metric[wrd] to remain directly comparable to XMoverScore which is
based on \mbert. Secondly, in our own experience, vanilla \mbert{} is very
robust in terms of layer choice, especially compared to vanilla \xlmr.
Intuitive choices like the first or last layer work very well for a lot of
problems. This is an important property for unsupervised metrics, since we
can’t easily justify a (supervised) hyperparameter search in an unsupervised
setting to determine the best layer or even a linear combination of those.

\section{Supplementary Data and Results}\label{sec:supplementary}
Table~\ref{table:pseudo-parallel} shows examples of pseudo-parallel data
obtained with \metric[wrd] and \metric[snt].
%
Tables~\ref{tab:newstest-2016-pearson},~\ref{tab:newstest-2017-pearson},~%
\ref{tab:mlqe-pearson}, and~\ref{tab:mqm-newseval4nlp-pearson} show
segment-level \pearson{} correlations with human judgments on WMT-16, WMT-17,
MLQE-PE, as well as WMT-MQM and Eval4NLP, respectively.
%
Table~\ref{tab:dataset-statistics} provides additional statistics for each
dataset.

A surprising finding is the poor performance of \metric[snt] and \distilscore{}
on the German-English language pair in
Table~\ref{tab:mqm-newseval4nlp-pearson}. It is well known that high-resource
language directions, such as English-German, can be affected by a lack of
low-quality translations~\citep{Fomicheva2020MLQEPEAM}, and with only
high-quality translations available, there is little variation in the scores,
which makes a meaningful assessment of correlation
difficult~\citep{Specia2020FindingsOT}. Further, since both \metric[snt] and
\distilscore{} are based on sentence embeddings of \xlmr{}, and sentence
embedding-based metrics are known to be a bit worse on average than their word
embedding-based counterparts, we believe that both aspects combined could be
the root cause for this.

\begin{table*}[htb]
    \centering
    \begin{tabularx}{\textwidth}{lXX}
    \toprule
         \textbf{Case} & \textbf{Source} & \textbf{Target}\\ \midrule
         Top-WRD & Uruguay belegt mit vier Punkten nur Platz Sieben. & Russia was second with four gold and 13 medals. \\
         Top-WRD & Soweit lautet zumindest die Theorie. & That, at least, is the theory.\\
         Rnd-WRD & Die USA stellen etwa 17.000 der insgesamt 47.000 ausländischen Soldaten in Afghanistan. & Currently, there are about 170,000 U.S. troops in Iraq and 26,000 in Afghanistan.\\
         Rnd-WRD & ``Das ist eine schwierige Situation'', sagte Kaczynski. & ``It seemed like a ridiculous situation,'' Vanderjagt said.\\
         \midrule
         Top-SNT & Die Wahlen für ein neues Parlament sollen dann Anfang Januar stattfinden. & 	Parliamentary elections are to be held by January.\\
         Top-SNT & Anzeichen für die Blauzungenkrankheit sind Fieber, Entzündungen und Blutungen an der Zunge der Tiere.	& Contact with the creatures can cause itching, rashes, conjunctivitis and, in some cases, breathing problems.\\
         Rnd-SNT & Riesen-Wirbel an der Universität Zagreb: An der wirtschaftlichen Fakultät und am Institut für Verkehrsstudien durchsuchen Polizisten die Büros von Dozenten.	& Those attending the Soil Forensics International Conference work in the fields of science, policing, forensic services as well as private industries.\\
         Rnd-SNT & Frankfurt soll WM-Finale der Frauen ausrichten &	The women's tournament gets underway on Sunday.\\
         \bottomrule
    \end{tabularx}
    \caption{Pseudo-parallel data obtained via \metric[wrd] and \metric[snt];
      top and random sentence pairs. The mined sentences are semantically
      similar, but contain factuality errors (e.g., have wrong places or
      numbers in hypotheses).}%
    \label{table:pseudo-parallel}
\end{table*}

\begin{table*}[htb]
  \centering
  \begin{tabular}{cllllllll}
    \toprule
    & \textbf{Metric} & de-en & en-ru & ru-en & ro-en & cs-en & fi-en & tr-en\\
    \midrule\multirow{3.5}{*}{\makecell{\faint{\textbf{\type{1/2}}}\\\faint{\textbf{Supervised}}}}
    & \faint{\monotransquest} & \faint{61.65} & \faint{66.69} & \faint{63.32} & \faint{62.36} & \faint{67.67} & \faint{68.33} & \faint{62.71}\\
    & \faint{\cometqe}          & \faint{65.73} & \faint{71.91} & \faint{69.71} & \faint{66.40} & \faint{67.98} & \faint{64.83} & \faint{53.73}\\
    \arrayrulecolor{gray}\cmidrule(l){2-9}\arrayrulecolor{black}
    & \faint{\bleu}           & \faint{45.39} & \faint{55.08} & \faint{46.33} & \faint{47.09} & \faint{53.80} & \faint{39.92} & \faint{47.15}\\

    \midrule\multirow{5}{*}{\makecell{\textbf{\type{3}}\\\textbf{Supervised}}}
    & \xmoverscore[UMD]   & 43.46 & 62.16 &\textbf{60.52}& 47.88 & 58.83 & 43.52 & 33.34\\
    & \xmoverscore[CLP]   & 45.29 & 63.58 & 56.12 & 54.24 & 58.89 & 51.40 & 42.14\\
    & \sentsim[BERTScore] & 48.49 & 50.37 & 57.89 & 55.06 & 59.08 & 46.66 &\textbf{45.47}\\
    & \sentsim[WMD]       & 47.78 & 48.49 & 56.19 & 54.48 & 56.87 & 46.00 &44.84\\
    & \distilscore{}      & 40.62 & 41.21 & 43.16 & 51.22 & 49.51 & 39.65 & 41.14\\

    \midrule\multirow{8}{*}{\textbf{Unsupervised}}
    & \metric[wrd]                & 48.94 & 60.97 & 59.09 & 56.06 & 57.15 & 53.76 & 41.15\\
    & \metric[snt]                & 30.48 & 39.73 & 35.31 & 44.18 & 40.80 & 31.30 & 30.62\\
    & \metric[wrd\,$\oplus$\,snt] &\textbf{50.37}& 62.92 & 60.49 & 60.07 &\textbf{59.25}& 52.93 & 44.41\\
    \cmidrule(l){2-9}
    & \metric[wrd][+]                & 48.97 & 60.57 & 58.35 & 56.23 & 56.44 & 53.78 & 41.30\\
    & \metric[wrd\,$\oplus$\,snt][+] & 50.29 & 62.37 & 59.43 &\textbf{60.71}& 58.47 & 51.48 & 44.19\\
    \cmidrule(l){2-9}
    & \metric[wrd][++]                & 44.50 & 61.45 & 53.50 & 56.03 & 52.95 & 54.08 & 40.65\\
    & \metric[wrd\,$\oplus$\,snt][++] & 47.27 &\textbf{64.14}& 56.40 & 60.36 & 56.29 &\textbf{55.62}& 44.85 \\
    \bottomrule
  \end{tabular}
  \caption{Segment-level \pearson{} correlations with human judgments on the WMT-16 dataset.}%
  \label{tab:newstest-2016-pearson}
\end{table*}

\begin{table*}[htb]
  \centering
  \begin{tabular}{cllllllll}
    \toprule
    & \textbf{Metric} & cs-en & de-en & fi-en & lv-en & ru-en & tr-en & zh-en\\
    \midrule\multirow{3.5}{*}{\makecell{\faint{\textbf{\type{1/2}}}\\\faint{\textbf{Supervised}}}}
    & \faint{\monotransquest} & \faint{60.93} & \faint{63.54} & \faint{65.33} & \faint{72.01} & \faint{59.56} & \faint{75.91} & \faint{68.03}\\
    & \faint{\cometqe}          & \faint{68.99} & \faint{69.34} & \faint{72.83} & \faint{64.75} & \faint{69.06} & \faint{68.43} & \faint{68.01}\\
    \arrayrulecolor{gray}\cmidrule(l){2-9}\arrayrulecolor{black}
    & \faint{\bleu}           & \faint{41.22} & \faint{41.29} & \faint{56.48} & \faint{39.28} & \faint{45.99} & \faint{53.06} & \faint{51.75}\\

    \midrule\multirow{5}{*}{\makecell{\textbf{\type{3}}\\\textbf{Supervised}}}
    & \xmoverscore[UMD]   & 41.72 & 51.19 &        56.61 & 56.11 &        47.24 & 46.52 & 57.73\\
    & \xmoverscore[CLP]   & 47.76 & 50.04 & 62.22 & 63.95 &        48.79 & 52.97 & 59.88 \\
    & \sentsim[BERTScore] & 49.90 & 52.26 &        57.85 & 57.42 &\textbf{55.10}& 56.84 & 59.59\\
    & \sentsim[WMD]       & 47.62 & 50.42 &        56.59 & 56.91 &        53.42 & 56.24 & 58.86\\
    & \distilscore{}      & 46.42 & 45.64 &        54.03 & 55.51 &        54.13 & 54.04 & 50.89\\

    \midrule\multirow{8}{*}{\textbf{Unsupervised}}
    & \metric[wrd]                & 46.70 & 52.71 & 61.91 & 59.22 & 49.10 & 50.06 & 54.95\\
    & \metric[snt]                & 38.89 & 41.92 & 39.77 & 48.95 & 37.27 & 48.83 & 43.10\\
    & \metric[wrd\,$\oplus$\,snt] &\textbf{50.67}&\textbf{56.50}& 61.86 & 64.54 & 53.17 & 57.31 & 58.80\\
    \cmidrule(l){2-9}
    & \metric[wrd][+]                & 44.55 & 52.96 & 60.96 & 59.02 & 48.82 & 49.70 & 54.75\\
    & \metric[wrd\,$\oplus$\,snt][+] & 48.62 & 56.31 & 60.44 & 63.62 & 54.19 &\textbf{57.54}&\textbf{60.28}\\
    \cmidrule(l){2-9}
    & \metric[wrd][++]                & 45.41 & 48.00 & 61.33 & 60.64 & 49.65 & 47.06 & 50.00\\
    & \metric[wrd\,$\oplus$\,snt][++] & 49.27 & 52.20 &\textbf{63.10}&\textbf{66.64}& 53.70 & 54.93 & 55.62\\
    \bottomrule
  \end{tabular}
  \caption{Segment-level \pearson{} correlations with human judgments on the WMT-17 dataset.}%
  \label{tab:newstest-2017-pearson}
\end{table*}

\begin{table*}[htb]
  \centering
  \begin{tabular}{cllllllll}
    \toprule
    & \textbf{Metric} & en-de & en-zh & ru-en & ro-en & et-en & ne-en & si-en\\
    \midrule\multirow{2}{*}{\makecell{\faint{\textbf{\type{1}}}\\\faint{\textbf{Supervised}}}}
    & \faint{\monotransquest} & \faint{41.85} & \faint{45.76} & \faint{76.76} & \faint{88.81} & \faint{73.19} & \faint{75.70} & \faint{61.90}\\
    & \faint{\cometqe}          & \faint{36.03} & \faint{30.70} & \faint{49.33} & \faint{64.95} & \faint{63.45} & \faint{57.46} & \faint{47.85}\\

    \midrule\multirow{5}{*}{\makecell{\textbf{\type{3}}\\\textbf{Supervised}}}
    & \xmoverscore[UMD]   &        16.56 &        16.48  &        28.07  &        65.83 &        53.95 &        38.23 &        18.81 \\
    & \xmoverscore[CLP]   & 25.59 &        20.25  &        20.31  &        57.34 &\textbf{58.46}&        25.15 &        16.74 \\
    & \sentsim[BERTScore] &         6.15 &        22.23  & 47.30 &\textbf{78.55}&        55.09 &\textbf{57.09}&\textbf{51.14}\\
    & \sentsim[WMD]       &         3.86 & 22.62 &\textbf{47.46} & 77.72 &        54.60 & 57.00 & 49.79 \\
    & \distilscore{}      &        12.96 &\textbf{28.68} &        45.34  &        76.57 &        51.16 &        46.73 &        41.76 \\

    \midrule\multirow{8}{*}{\textbf{Unsupervised}}
    & \metric[wrd]                & 24.53 & 21.58 & 16.66 & 60.30 & 54.83 & 28.62 & 11.38\\
    & \metric[snt]                & 13.62 & 13.27 & 39.09 & 66.50 & 41.75 & 46.83 & 41.49\\
    & \metric[wrd\,$\oplus$\,snt] & 24.67 & 21.63 & 27.83 & 71.48 & 57.62 & 45.70 & 35.25\\
    \cmidrule(l){2-9}
    & \metric[wrd][+]                & 23.78 & 21.40 & 15.18 & 60.39 & 56.27 & 27.34 & 12.22\\
    & \metric[wrd\,$\oplus$\,snt][+] & 22.00 & 21.41 & 27.71 & 73.65 & 57.94 & 47.27 & 39.91\\
    \cmidrule(l){2-9}
    & \metric[wrd][++]                & 26.17 & 27.16 & 0.75 & 32.92 & 52.24 & 12.79 & 14.30\\
    & \metric[wrd\,$\oplus$\,snt][++] &\textbf{26.37}& 27.26 & 9.29 & 57.70 & 56.81 & 31.24 & 30.38\\
    \bottomrule
  \end{tabular}
  \caption{Segment-level \pearson{} correlations with human judgments on the MLQE-PE dataset.}%
  \label{tab:mlqe-pearson}
\end{table*}

\begin{table*}[htb]
  \centering
  \begin{tabular}{clllll}
    \toprule
    & & \multicolumn{2}{c}{\textbf{WMT-MQM}} & \multicolumn{2}{c}{\textbf{Eval4NLP}}\\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}
    & \textbf{Metric} & en-de & zh-en & de-zh & ru-de\\
    \midrule\multirow{3.5}{*}{\makecell{\faint{\textbf{\type{1/2}}}\\\faint{\textbf{Supervised}}}}
    & \faint{\monotransquest} & \faint{31.38} & \faint{53.07} & \faint{34.66} & \faint{49.76}\\
    & \faint{\cometqe}          & \faint{40.94} & \faint{50.84} & \faint{33.51} & \faint{46.49}\\
    \arrayrulecolor{gray}\cmidrule(l){2-6}\arrayrulecolor{black}
    & \faint{\bleu}           & \faint{17.94} & \faint{21.58} & \faint{ --- } & \faint{ --- }\\

    \midrule\multirow{5}{*}{\makecell{\textbf{\type{3}}\\\textbf{Supervised}}}
    & \xmoverscore[UMD]   & 12.72 & 27.41 &  10.85 &        48.35 \\
    & \xmoverscore[CLP]   & 12.89 & 28.29 &  21.61 &        52.25 \\
    & \sentsim[BERTScore] &  1.03 & 26.39 &  -7.71 &\textbf{60.91}\\
    & \sentsim[WMD]       & -0.23 & 24.70 & -11.54 & 60.42 \\
    & \distilscore{}      & -2.66 &  7.06 &   6.57 &        51.22 \\

    \midrule\multirow{8}{*}{\textbf{Unsupervised}}
    & \metric[wrd]                & 18.13 &\textbf{28.43}& 29.29 & 44.63\\
    & \metric[snt]                & -5.93 &  4.99 &  0.86 & 39.91\\
    & \metric[wrd\,$\oplus$\,snt] &        13.94 &        25.17 &        24.66 & 55.08\\
    \cmidrule(l){2-6}
    & \metric[wrd][+]                & 19.83 & 26.46 & 29.99 & 42.59\\
    & \metric[wrd\,$\oplus$\,snt][+] & 13.72 & 21.7  & 22.64 & 53.8 \\
    \cmidrule(l){2-6}
    & \metric[wrd][++]                &\textbf{20.19}& 17.80 &\textbf{36.51}& 14.32\\
    & \metric[wrd\,$\oplus$\,snt][++] & 17.18 & 16.97 & 34.00 & 30.09\\
    \bottomrule
  \end{tabular}
  \caption{Segment-level \pearson{} correlations with human judgments on the WMT-MQM and Eval4NLP datasets.}%
  \label{tab:mqm-newseval4nlp-pearson}
\end{table*}

\begin{table*}[htb]
  \centering
  \begin{tabular}{lllll}
  \begin{tabular}{lllll}
    \toprule
    Dataset  & Pairs & Tokens & Type\\
    \midrule
      WMT-16 &   560 &   9886 &   CA\\
      WMT-17 &   560 &  11189 &   CA\\
     MLQE-PE &  1000 &  15263 & CLDA\\
    Eval4NLP &  1295 &  25975 & CLDA\\
     WMT-MQM & 17090 & 549835 &  MQM\\
    \bottomrule
  \end{tabular}
  \end{tabular}
  \caption{Statistics of our used datasets averaged over language pairs. For
  each dataset we report the number of sentences we evaluated on, the amount of
  tokens in these, and the type of human annotation. The number of tokens
  refers to source sentences.}%
  \label{tab:dataset-statistics}
\end{table*}


